Online Demand Scheduling with Failovers

Motivated by cloud computing applications, we study the problem of how to optimally deploy new hardware subject to both power and robustness constraints. To model the situation observed in large-scale data centers, we introduce the Online Demand Scheduling with Failover problem. There are $m$ identical devices with capacity constraints. Demands come one-by-one and, to be robust against a device failure, need to be assigned to a pair of devices. When a device fails (in a failover scenario), each demand assigned to it is rerouted to its paired device (which may now run at increased capacity). The goal is to assign demands to the devices to maximize the total utilization subject to both the normal capacity constraints as well as these novel failover constraints. These latter constraints introduce new decision tradeoffs not present in classic assignment problems such as the Multiple Knapsack problem and AdWords. In the worst-case model, we design a deterministic $\approx \frac{1}{2}$-competitive algorithm, and show this is essentially tight. To circumvent this constant-factor loss, which in the context of big cloud providers represents substantial capital losses, we consider the stochastic arrival model, where all demands come i.i.d. from an unknown distribution. In this model we design an algorithm that achieves a sub-linear additive regret (i.e. as OPT or $m$ increases, the multiplicative competitive ratio goes to $1$). This requires a combination of different techniques, including a configuration LP with a non-trivial post-processing step and an online monotone matching procedure introduced by Rhee and Talagrand.

==> offline_max_util.tex <==
\section{Offline Utilization Maximization}\label{sec_off_max_util}

In this section, we again begin with a failover capacity $B \geq 1$ and a collection of jobs with sizes in $[0, \min(0, \frac{B}{2})]$ such that we need to assign jobs to pairs of machines satisfying both the normal and failover constraints. Previously, we were interested minimizing the number of machines needed to assign all jobs. Now we consider the utilization maximization variant, where we are given a number of machines $m \geq 2$, and we assign some subset of jobs to $m$ machines to maximize the utilization (the total size of all assigned jobs.)

By a similar configuration LP, $\lpconfigmax$, and rounding, we give an efficient offline algorithm for this problem with small additive regret.

\begin{thm}\label{thm_main_off_max}
	There exists an efficient algorithm that, given failover capacity $B \geq 1$, a collection of jobs, and number of machines $m \geq 2$, achieves utilization at least $\big(1 - O(\epsilon)\big) \opt(\lpconfigmax) - O(\frac{1}{\epsilon^5}) \geq \big(1 - O(\epsilon)\big) \opt - O(\frac{1}{\epsilon^5})$ machines for any $\epsilon \in (0,1)$.
\end{thm}

\subsection{Configuration LP Rounding}

The LP we consider is the natural maximization configuration LP. For any configuration $c$, we define $s(c) = \sum_{j \in c} s_j$ to the total size of all jobs in $c$.

\begin{equation}\tag{$\lpconfigmax$}\label{eq_lpconfigmax}
	\begin{array}{rrll}
		\max & \frac{1}{2}\sum_c s(c) \cdot x_c\\
		s.t. & \sum_c n_t(c) \cdot x_c & \leq 2 n_t &\quad \forall t\\
		& \sum_c x_c &\leq m\\
		& x & \geq 0
	\end{array} 
\end{equation}

Similar to $\lpconfigmin$, this LP is a relaxation of our utilization maximization problem by considering the natural setting the $x$-variables defined by an assignment of job to machines, and it can be approximately solved via column generation.

\begin{lemma}\label{lem_lpconfigmax_relax}
	For any collection of jobs $J$, we have $\opt \big( \lpconfigmax(J) \big) \geq \opt(J)$.
\end{lemma}

\begin{lemma}\label{lem_lpconfigmax_solve}
	We can efficiently solve $\lpconfigmax$ to obtain an extreme point with objective value at least $\opt(\lpconfigmax) - error$. \rnote{to prove}
\end{lemma}

Further, $\lpconfigmax$ only has $T+1$ non-trivial constraints, so every extreme point of $\lpconfigmax$ has at most $T+1$ non-zero variables. Instead of rounding these variables up, we instead round them down, giving the next lemma. Note that we use the fact that $s(c) \leq 1$ for every configuration $c$.

\begin{lemma}\label{lem_lpconfigmax_round}
	Given an extreme point of $\lpconfigmax$ with objective value $U$, rounding down all fractional variables to the next smallest integer gives an integral solution to $\lpconfigmax$ with objective value at least $U - \frac{T+1}{2}$.
\end{lemma}

Using the same algorithm to turn a collection of configurations into a job assignment (\Cref{thm_config_match}), we can obtain an assignment by losing only $O(DT)$ utilization.

\begin{lemma}\label{lem_config_match_max}
	Let $m \geq 2$. Given a collection $C$ of at most $m$ configurations with total utilization $U$ (defined as $\frac{1}{2} \sum_{c \in C} s(c)$), we can efficiently assign at most $\frac{1}{2} \sum_{c \in C} n_t(c)$ jobs of type $t$ for all $t$ to the edges of $m$ machines with total utilization at least $U - O(DT)$, where there at most $T$ job types and at most $D$ jobs in any configuration.
\end{lemma}
\begin{proof}
	Our algorithm is the following: We remove an arbitrary $O(DT)$ configurations from $C$ to obtain sub-collection $C' \subset C$. Then, we run the algorithm \matchalg~ on $C'$. This completes the description of the algorithm.
	
	By \Cref{thm_config_match}, this algorithm is efficient and assigns $\frac{1}{2} \sum_{c \in C'} d_t(c) \leq \frac{1}{2} \sum_{c \in C} d_t(c)$ jobs of type $t$ for all $t$ to at most $\lvert C' \rvert + O(DT) \leq m - O(DT) + O(DT) \leq m$ machines. Because we removed $O(DT)$ configurations from $C$ to obtain $C'$, the total utilization of this assignment is at least $U - O(DT)$, as required.
\end{proof}

It remains to modify the input jobs to obtain a sub-instance where $D$ and $T$ are both small. To achieve this, we again use linear grouping on the medium jobs and group the small jobs into blocks.

\subsection{Handling small and large jobs}

\subsection{Putting it all together}

==> offline_min_machines.tex <==
\section{Offline Machine Minimization}\label{sec_offline_min_machines}

The goal of this section is to solve the following machine minimization problem: Given a failover capacity $B \geq 1$ and a collection of jobs such that job $j$ has size $s_j \in [0, \min(1, \frac{B}{2})]$, the goal is to assign each job to a pair of machines satisfying:
\begin{enumerate}
	\item (Normal Constraint) For every machine $u$, we have $L_u = \sum_{v \neq u} L_{uv} \leq 1$, where we define $L_{uv} = \sum_{j \rightarrow uv} s_j$ to be the total load on ``edge'' uv (i.e. all jobs assigned to the pair of machines $uv$.)
	\item(Failover Constraint) For every machine $u$, we have $L_u + \max_{v \neq u} L_{uv} \leq B$.
\end{enumerate}
We want to minimize the number of machines needed to assign all jobs subject to the above constraints.

The main result of this section is an efficient offline algorithm for this problem with small additive regret.

\begin{thm}\label{thm_main_off_min}
	There exists an efficient algorithm that, given failover capacity $B \geq 1$ and a collection of jobs, assigns the jobs using most $\big(1 + O(\epsilon)\big) \opt(
	\lpconfigmin) + O(\frac{1}{\epsilon^5}) \leq \big(1 + O(\epsilon)\big) \opt + O(\frac{1}{\epsilon^5})$ machines for any $\epsilon \in (0,1)$.
\end{thm}

Our algorithm is based on rounding a configuration linear program (LP), $\lpconfigmin$, which we define in the next section, similar to the Gomory-Gilmore LP for bin packing.

\subsection{Configuration LP}

Consider a fixed packing of the jobs into some number of machines. We can view the collection of jobs assigned to the edges incident to each machine as a configuration. Precisely, we define a \emph{configuration} to be a collection of jobs $c$ such that $\sum_{j \in c} s_j \leq 1$ and $\sum_{j \in c} s_j + \max_{j \in c} s_j \leq B$. Note that the first constraint is exactly the normal constraint, while the second is a relaxation of the failover constraint, because the most-loaded edge incident on some machine can be larger than the single largest job assigned to that machine. Thus, our notion of configuration does not take in to account how the jobs are assigned to the respective edges incident on each machine.

To define our configuration LP, we suppose the input collection of jobs is partitioned into $T$ \emph{job types} such that type $t$ consists of $n_t$-many jobs each with size $s_t$. Thus each configuration $c$ is defined by a number $n_t(c) \in \mathbb{N}$ of jobs for each type $t$ such that $\sum_t n_t(c) \cdot s_t \leq 1$ and $\sum_t n_t(c) \cdot s_t + \max_{t \mid\, n_t(c) > 0} s_t \leq B$. We are ready to define our configuration LP:

    \begin{equation}\tag{$\lpconfigmin$}\label{eq_lpconfigmin}
		\begin{array}{rrll}
			\min & \sum_c x_c\\
			s.t. & \sum_c n_t(c) \cdot x_c & \geq 2 n_t &\quad \forall t\\
			& x & \geq 0
		\end{array} 
	\end{equation}

It is immediate that $\lpconfigmin$ is a relaxation of our problem by taking the natural setting of the $x$-variables defined by a feasible assignment to machines: let $x_c$ be the number of machines whose collection of jobs assigned to its edges are exactly those in $c$. Every machine defines a feasible configuration this way. Thus the next lemma is immediate. For any collection of jobs $J$, we let $\lpconfigmin(J)$ denote the configuration LP for this collection of jobs; $\opt(J)$ is defined analogously.

\begin{lemma}\label{lem_lpconfigmin_relax}
	For any collection of jobs $J$, we have $\opt \big( \lpconfigmin(J) \big) \leq \opt(J)$.
\end{lemma}

Although $\lpconfigmin$ has exponentially many variables in general, we can approximately solve it via column generation.

\begin{lemma}\label{lem_lpconfigmin_solve}
	We can efficiently solve $\lpconfigmin$ to obtain an extreme point with objective value at most $\opt(\lpconfigmin) + error$. \rnote{to prove}
\end{lemma}

Further, observe that $\lpconfigmin$ only has $T$ non-trivial constraints, so every extreme point of $\lpconfigmin$ has at most $T$ non-zero variables. This is because all but at most $T$ constraints are the non-negativity constraints in any basis defining this extreme point. Thus, the next lemma is immediate.

\begin{lemma}\label{lem_lpconfigmin_round}
	Given an extreme point of $\lpconfigmin$ with objective value $N$, rounding up all fractional variables to the next largest integer gives an integral solution to $\lpconfigmin$ with objective value at most $N + T$.
\end{lemma}

To summarize this section, we can efficiently obtain a collection of configurations, each corresponding to a machine, that ``covers'' all the jobs. However, these configurations do not specify how to actually assign the jobs to the edges incident on the corresponding machine. This is the goal of the next section.

\subsection{Matching configurations}

Suppose we are given a collection of $N$ configurations. Our goal in this section is to realize these configurations by actually assigning jobs to edges. The main challenge is maintaining the failover constraint.

Consider a fixed configuration. Regardless of how we assign the jobs of that configuration to this machine's edges, the normal constraint will be satisfied by definition of configuration.  This is not the case for the failover constraint. Recall that the definition of configuration only gives us that $\sum_{j \in c} s_j + \max_{j \in c} s_j \leq B$. To ensure that our algorithm assigns the jobs satisfying the failover constraint, it suffices to ensure that we assign at most one job per edge. It is not clear that such a near-optimal assignment should even exist, but the main result of this section is that - by opening slightly more machines - we can find such an assignment that realizes any given collection of configurations satisfying both the normal- and failover constraints.

\begin{thm}\label{thm_config_match}
	Given any collection $C$ of $N$ configurations such that there at most $T$ job types and at most $D$ jobs in any configuration, we can efficiently assign $\frac{1}{2} \cdot \sum_{c \in C} n_t(c)$ jobs of type $t$ for all $t$ to the edges of $N + O(DT)$ machines satisfying both the normal- and failover constraints.
\end{thm}

We will need the following subroutine to assign some jobs outside of their respective configurations.

\begin{lemma}\label{lem_matching_unit}
	Consider any collection of jobs with total size at most $S \geq 1$. We can efficiently assign these jobs to the edges of $8 \cdot S + 1$ machines satisfying both the normal- and failover constraints.\rnote{this can probably be improved/ simplified}
\end{lemma}
\begin{proof}
	Our algorithm will only open edges - that is, we will open machines in pairs and will only assign jobs to the edges of the paired machines. Our algorithm is the following: Consider jobs in any order. Assign each job to already-opened edge as long as the normal- and failover constraints remain satisfied. Else open a new edge and assign the job there.
	
	It is clear that the algorithm is efficient and satisfies the constraints. We claim this algorithm opens at most $8 \cdot S + 2$ machines (i.e. $4 \cdot S + 1$ edges) at most. To see this, note that every edge except at most one has load at least $\frac{1}{4}$. If not, then consider the first time that there are two open edges with load less than $\frac{1}{4}$. It must be the case that the last job the algorithm considered had size less than $\frac{1}{4}$, but the algorithm decided to open a new edge for this job rather than assign it to a previous edge that already had load less than $\frac{1}{4}$. This contradicts the definition of the algorithm.
\end{proof}

The algorithm guaranteed by \Cref{thm_config_match} is a simple greedy algorithm.

\medskip
\hrule
\smallskip
\hrule
\smallskip
\matchalg: Given collection $C$ of configurations, we assign them to edges as follows:
\begin{enumerate}
	\item Open $N$ machines - one corresponding to each configuration in $C$.
	\item Consider job types in arbitrary order $t = 1, \dots, T$.
	\item When considering job type $t$, partition the configurations $C = L_t \cup R_t$ such that their total $t$-degrees, so $\sum_{c \in L_t} d_t(c)$ and  $\sum_{c \in R_t} d_t(c)$, differ by at most $D_t$. We define $D_t$ to be the maximum number of type $t$ jobs in any configuration. (This can be achieved, e.g., by initializing $L_t, R_t = \emptyset$, and adding configurations one-by-one to the set with minimum total $t$-degree.)
	\item Given this partition, as long as there exists a configuration $c \in L_t$ that is currently assigned less than $d_t(c)$ jobs of type $t$, we pick such a configuration and assign a job of type $t$ on an arbitrary edge from $c$ to $c' \in R_t$ that has not yet been assigned a job and $c'$ is currently assigned less than $d_t(c')$ jobs of type $t$. If no such edge exists, then we stop and move on to the next job type.\label{step_one_per_edge}
	\item Once we are done considering all job types, let $a_t(c)$ be the number of jobs of type $t$ assigned to edges incident on configuration $c$. Then, we assign the remaining $d_t(c) - a_t(c)$ jobs for every type $t$ and configuration $c$ using \Cref{lem_matching_unit}.\label{step_unassigned}
\end{enumerate}
\medskip
\hrule
\smallskip
\hrule
\medskip

\begin{proof}[Proof of \Cref{thm_config_match}]
	It is clear that \matchalg~ is efficient. The total number of type $t$ jobs assigned by the algorithm is exactly $\frac{1}{2} \sum_c a_t(c) + \sum_c \big(d_t(c) - a_t(c) \big) \geq \frac{1}{2} \sum_c d_t(c)$. Further, this assignment satisfies both the normal- and failover constraints, because we assign at most one job per edge in Step \ref{step_one_per_edge}, and for all remaining jobs, \Cref{lem_matching_unit} ensures the constraints are satisfied.
	
	It remains to show that we open $N + O(DT)$ machines. In particular, by \Cref{lem_matching_unit} it suffices to show that the total size of all unassigned jobs in Step \ref{step_unassigned} is $O(DT)$. When considering job type $t$, there are two possibilities:
	\begin{enumerate}
		\item The algorithm assigns $d_t(c)$ type $t$ jobs to each $c \in L_t$: Thus, we assign $\sum_{c \in L_t} d_t(c)$ type $t$ jobs to edges between $L_t$ and $R_t$. Recall that the initial total $t$-degrees of $L_t$ and $R_t$ differ by at most $D_t$, so there are at most $D_t$ remaining unassigned $t$-degrees in $R_t$. The total size of these jobs it at most $1$ (because $D_t$ jobs of type $t$ form a valid configuration.) This contributes total size $O(T)$ over all job types.
		\item The algorithm fails to assign a job of type $t$ from a configuration $c \in L_t$ to $R_t$: In this case, every edge from $c$ to some $c' \in R_t$ either is already assigned some job or $c'$ has already been assigned $d_t(c')$ jobs of type $t$. Note that there can be at most $D$ configurations satisfying the former, each with remaining $t$-degree at most $D_t$, and all other configurations in $R_t$ have zero remaining $t$-degree. We conclude, the total remaining $t$-degree in $L_t$ and $R_t$ is $O(D \cdot D_t)$, which contributes $O(D)$ total size. This contributes total size $O(DT)$ over all job types.
	\end{enumerate}
	We conclude, the total size of all unassigned jobs is $O(DT)$, as required.
\end{proof}

We summarize the main results of this section and the previous with the next theorem.

\begin{thm}\label{thm_lpconfig_main}
	For any collection of jobs $J$ such that there are at most $T$ jobs types and at most $D$ jobs in any configuration, we can efficiently assign the jobs to $\opt(\lpconfigmin) + O(DT) + error$ machines satisfying both the normal and failover constraints.
\end{thm}
\begin{proof}
	Our algorithm is to solve $\lpconfigmin$ up to additive error $error$ by \Cref{lem_lpconfigmin_solve}. Then we round $\lpconfigmin$ by \Cref{lem_lpconfigmin_round} to obtain an integral solution and thus a collection of at most $\opt(\lpconfigmin) + T + error$ configurations $C$ such that $\sum_{c \in C} d_t(c) \geq 2 n_t$ for all types $t$. Applying the algorithm guaranteed by \Cref{thm_config_match} to these configurations opens at most the desired number of machines and assigns at least $\frac{1}{2} \cdot \sum_{c \in C} n_t(c) \geq n_t$ jobs of type $t$ for all $t$ (i.e. we can assign all jobs in $J$.)
\end{proof}

To obtain our main result, \Cref{thm_main_off_min}, it remains to show how to take $D, T$ both small enough. We do so in the next section by handling the small and large jobs separately and rounding the sizes of the remaining ``medium'' jobs. 

\subsection{Handling small and large jobs}\rnote{to check; maybe sloppy?}\label{sec_small_large_jobs}

Given a collection of jobs $J$ and parameter $\epsilon \in (0,1)$, we partition $J = S \cup M$ into small ($s_j < \epsilon^2$) and medium jobs ($s_j \geq \epsilon^2$), respectively.

For the small jobs $S$, we group them into \emph{blocks} of size $\epsilon$. To achieve this, let $\tilde{S}$ be a collection of $\lceil \frac{1}{\epsilon} \sum_{j \in S} s_j \rceil$ jobs each of size $\epsilon$. Our configuration LP will not assign small jobs individually - rather we will assign blocks of small jobs, correspond to jobs in $\tilde{S}$.

For the medium jobs $M$, we do linear grouping with $\frac{1}{\epsilon^3}$ groups: Let $n = \lvert M \rvert$. Partition $M$ into $\frac{1}{\epsilon^3}$ groups, consisting of the $\epsilon^3 n$ largest jobs, the next $\epsilon^3 n$ largest jobs, and so on. Note every group has size exactly $\epsilon^3 n$ except possibly the last group, corresponding to the smallest jobs. At this point, let $L$ be the first group, corresponding to the largest jobs. We can now partition $J = S \cup (M \setminus L) \cup L$. For the remaining groups of jobs in $M \setminus L$, let $\tilde{M}$ denote the modified set of jobs, where we round the size of each job in $M \setminus L$ up to the largest size in its group. This completes the description of linear grouping.

To summarize, we have three collections of jobs: blocks of small jobs $\tilde{S}$ such that each block has size exactly $\epsilon$, grouped medium jobs $\tilde{M}$ with sizes at least $\epsilon^2$ and a $O(\frac{1}{\epsilon^3})$ distinct job sizes (by the final rounding), and large jobs $L$ with sizes at least $\epsilon^2$ such that there are at most $\epsilon^3 \lvert M \rvert$ such jobs. We will handle the large jobs separately. For the blocks and grouped medium jobs, we will use the configuration LP. The next lemma states that our modifications of the small and medium jobs do not increase $\opt(\lpconfigmin)$ by much.

\begin{comment}
\begin{lemma}\label{lem_lin_group}
	Consider the linear grouping described above for jobs $M$ with $\frac{1}{\epsilon^3}$ groups for any $\epsilon \in (0,1)$. Then we have $\opt(\tilde{M}) \leq \opt(M)$. 
\end{lemma}
\begin{proof}
	Recall that $\tilde{M}$ is obtained from $M$ by excluding $L$ (the group of the largest $\epsilon^3 n$ jobs) and rounding up all remaining groups. Thus, for every group $G$ in $M$ except $L$, there exists a next-larger group $G'$ in $M$ with at least as many jobs such that every job in $G'$ has size larger than every job in $G$. This still holds after rounding up all job sizes in $G$ to largest job in $G$, which is how we obtain $\tilde{M}$. Thus, we conclude $\opt(\tilde{M}) \leq \opt(M)$.
\end{proof}
\end{comment}

\begin{lemma}\label{lem_small_med_lp}
	Let $\lpconfigmin(\tilde{S} \cup \tilde{M})$ be the configuration LP defined with one job type for all blocks and $O(\frac{1}{\epsilon^3})$ job types - one for each group in $\tilde{M}$. Then $\opt\big(\lpconfigmin(\tilde{S} \cup \tilde{M})\big) \leq \big(1 + O(\epsilon)\big) \opt \big(\lpconfigmin(J)\big)$.
\end{lemma}
\begin{proof}
	We first claim that $\opt \big( \lpconfigmin(S \cup \tilde{M}) \big)\leq \opt \big( \lpconfigmin(J) \big)$. To see this, recall that $\tilde{M}$ is obtained from $M$ by excluding $L$ (the group of the largest $\epsilon^3 n$ jobs) and rounding up all remaining groups. Thus, for every group $G$ in $M$ except $L$, there exists a next-larger group $G'$ in $M$ with at least as many jobs such that every job in $G'$ has size larger than every job in $G$. This still holds after rounding up all job sizes in $G$ to largest job in $G$, which is how we obtain $\tilde{M}$. Thus we have $\opt \big( \lpconfigmin(S \cup \tilde{M}) \big)\leq \opt \big( \lpconfigmin(J) \big)$.
	
	Using the above inequality, it suffices to show $\opt\big(\lpconfigmin(\tilde{S} \cup \tilde{M})\big) \leq \big(1 + O(\epsilon)\big) \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$. We will use an optimal solution for $\lpconfigmin(S \cup \tilde{M})$ to construct a feasible solution to $\lpconfigmin(\tilde{S} \cup \tilde{M})$ without increasing the objective value by much.
	
	To achieve this, we map each configuration of jobs $S \cup \tilde{M}$ to one using jobs $\tilde{S} \cup \tilde{M}$ as follows: Consider any configuration of jobs $S \cup \tilde{M}$. We keep all $\tilde{M}$ jobs. For the $S$ jobs, let $s$ be the total size of all small jobs in this configuration such that $s \in [k \cdot \epsilon, (k+1) \cdot \epsilon)$ for some $k = 0,1, 2, \dots$. We arbitrarily remove small jobs from this machine until the total size of the remaining small jobs lies in the interval $[k \cdot \epsilon - \epsilon^2, k \cdot \epsilon]$. In doing so, we remove at most $\epsilon + \epsilon^2$ units of small jobs (using the fact that every small job has size at most $\epsilon^2$.) Then we replace the $S$ jobs in this configuration with $\max(0, k-1)$ blocks of small jobs (i.e. jobs in $\tilde{S}$) to the configuration. This completes the description for the resulting configuration of jobs $\tilde{S} \cup \tilde{M}$.
	
	\begin{prop}
		The above procedure always creates a valid configuration.
	\end{prop}
	\begin{proof}
		Let $c$ be the input configuration of jobs $S \cup \tilde{M}$ and $c'$ the resulting configuration of jobs $\tilde{S} \cup \tilde{M}$. We need to show that $\sum_{j \in c'} s_j \leq 1$ and $\sum_{j \in c'} s_j + \max_{j \in c'} s_j \leq B$. For the first constraint, note that we only remove small jobs and then round down the remaining small size to obtain some number of blocks. Thus, we have $\sum_{j \in c'} s_j \leq \sum_{j \in c} s_j \leq 1$, so first constraint is satisfied.
		
		It remains to show the second constraint. There are two cases to consider.
		\begin{enumerate}
			\item If $k \leq 1$ (as defined in the above procedure), then $c'$ contains no blocks of small jobs. Thus, the only jobs in $c'$ are exactly the medium jobs of $c$. Then $\max_{j \in c'} s_j \leq \max_{j \in c} s_j$. We conclude, $\sum_{j \in c} s_j + \max_{j \in c} s_j \leq \sum_{j \in c} s_j + \max_{j \in c} s_j \leq B$ as required.
			\item Otherwise $k \geq 2$. In this case, $c'$ contains $k-1 \geq 1$ blocks. The total size of the small jobs in $c$ is at least $\epsilon$ larger than the total size of all blocks in $c'$. Thus, $\sum_{j \in c'} s_j \leq \sum_{j \in c}  -\epsilon$. Further, because every block has size exactly $\epsilon$, we have $\max_{j \in c'} s_j \leq \max\big(\max_{j \in c} s_j, \epsilon\big) \leq \max_{j \in c} + \epsilon$. Combining both bounds gives the desired result.
		\end{enumerate}
		We conclude, the configuration $c'$ satisfies both constraints.
	\end{proof}

\begin{comment}
	Consider an optimal assignment of jobs $S \cup \tilde{M}$ into $\opt(S \cup \tilde{M})$ machines. For each machine in this assignment, we turn it into a configuration as follows: For every job in $\tilde{M}$ assigned to an edge of this machine, we add one such job to the configuration. For the small jobs, let $s$ be the total size of all small jobs assigned to edges of this machine such that $s \in [k \cdot \epsilon, (k+1) \cdot \epsilon)$ for some $k = 0,1, 2, \dots$. We arbitrarily remove small jobs from this machine until the total size of the remaining small jobs lies in the interval $[k \cdot \epsilon - \epsilon^2, k \cdot \epsilon]$. In doing so, we remove at most $\epsilon + \epsilon^2$ units of small jobs (using the fact that every small job has size at most $\epsilon^2$.) Then we add $\max(0, k-1)$ blocks of small jobs to the configuration. This completes the description of each machine's configuration. 
	Note that for each configuration, the total size of all blocks is at most $2\epsilon + \epsilon^2 = O(\epsilon)$ less than than the total small size of the corresponding machine. Thus, over all configurations, the toal size of all blocks at least $\sum_{j \in S} s_j - O(\epsilon) \cdot \opt(S \cup \tilde{M})$.
	
	\begin{prop}
		The above procedure always creates a valid configuration.
	\end{prop}
	\begin{proof}
		Let $u$ be the machine and $c$ the resulting configuration. We need to show that $\sum_{j \in c} s_j \leq 1$ and $\sum_{j \in c} s_j + \max_{j \in c} s_j \leq B$. Note that we only remove jobs from the machine to create a configuration, so $\sum_{j \in c} s_j \leq L_u \leq 1$.
		
		It remains to show the second constraint. There are two cases to consider.
		\begin{enumerate}
			\item If $k \leq 1$ (as defined in the above procedure), then $c$ contains no blocks of small jobs. Thus, the only jobs in $c$ are exactly the medium jobs assigned to $u$. Then $\max_{j \in c} s_j = \max_{j \rightarrow uv \mid v \neq u} s_j \leq \max_{v \neq u} L_{uv}$. We conclude, $\sum_{j \in c} s_j + \max_{j \in c} s_j \leq L_u + \max_{v \neq u} L_{uv} \leq B$ as required.
			\item Otherwise $k \geq 2$. In this case, $c$ contains $k-1 \geq 1$ blocks. The total size of the small jobs assigned to $u$ is at least $\epsilon$ larger than the total size of all blocks in $c$. Thus, $\sum_{j \in c} s_j \leq L_u  -\epsilon$. Further, because every block has size exactly $\epsilon$, we have $\max_{j \in c} s_j \leq \max\big(\max_{j \rightarrow uv \mid v \neq u} s_j, \epsilon\big) \leq \max_{v \neq u} L_{uv} + \epsilon$. Combining both bounds gives the desired result.
		\end{enumerate}
		We conclude, the configuration $c$ satisfies both constraints.
	\end{proof}

	By the above procedure applied to each machine, we obtain $\opt(S \cup \tilde{M})$ feasible configurations of $\tilde{S} \cup \tilde{M}$ after removing some small jobs. We have assigned all $\tilde{M}$ jobs this way, so it remains to assign some number of blocks. Recall there are $\lceil \frac{1}{\epsilon} \sum_{j \in S} s_j \rceil$ blocks with total size at most $\sum_{j \in S} s_j + \epsilon$. The total size of all blocks in the configurations so far is at least $\sum_{j \in S} s_j - O(\epsilon) \cdot \opt(S \cup \tilde{M})$, so it remains to assign $O(\epsilon) \cdot \opt(S \cup \tilde{M})$ total size of blocks. We do so using an extra $O(\epsilon) \cdot \opt(S \cup \tilde{M})$ machines (and thus this many feasible configurations) by \Cref{lem_matching_unit}. Taking $x_c$ to be the number of copies of configuration $c$ used gives the desired solution.
\end{comment}
	Finally, we construct a feasible setting of the $x$-variables for $\lpconfigmin(\tilde{S} \cup \tilde{M})$ with objective value at most $\big(1 + O(\epsilon)\big) \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$, completing the proof. Let $x^*$ be an optimal solution for $\lpconfigmin(S \cup \tilde{M})$. Let $C$ be the collection of possible configurations for jobs $S \cup \tilde{M}$ and $C'$ the collection of possible configurations for jobs $\tilde{S} \cup \tilde{M}$. For every $c' \in C'$, we define $\bar{x}_{c'} = \sum_{c \in C \mid c \rightarrow c'} x^*_c$, where $c \rightarrow c'$ denotes the event that the above procedure maps configuration $c$ to $c'$. In words, we map the configurations chosen by $x^*$ in $C$ to configurations in $C'$. At this point, our objective value is $\sum_{c' \in C'} \bar{x}_{c'} = \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$. It remains to modify $\bar{x}$ so that it is feasible.
	
	Note that $\lpconfigmin(\tilde{S} \cup \tilde{M})$ and $\lpconfigmin(S \cup \tilde{M})$ have the same constraints for the medium jobs, and the mapping $c \rightarrow c'$ preserves the number of each type of medium job. Thus, $\bar{x}$ satisfies all medium job constraints. It remains to satisfy the constraint for the blocks.
	
	Recall there are $\lceil \frac{1}{\epsilon} \sum_{j \in S} s_j \rceil$ blocks with total size at most $\sum_{j \in S} s_j + \epsilon$. Thus, it suffices to ensure that the total size of blocks in $\bar{x}$ is at least $2 \sum_{j \in S} s_j + 2 \epsilon$. Note that for each mapping, $c \rightarrow c'$, the total size of all blocks in $c'$ is at most $2\epsilon + \epsilon^2 = O(\epsilon)$ less than than the total small size of $c$. Further, the total size of small jobs in $x^*$ is at least $2 \sum_{j \in S} s_j$ by the constraints of $\lpconfigmin(S \cup \tilde{M})$. It follows, currently the total size of blocks in $\bar{x}$ is at least $2 \sum_{j \in S} s_j - O(\epsilon) \cdot \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$. It remains to assign at $O(\epsilon) \cdot \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$ units of blocks. We do so using an extra $O(\epsilon) \cdot \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$ machines (and thus this many feasible configurations) by \Cref{lem_matching_unit}. Adding these $O(\epsilon) \cdot \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$-many configurations to $\bar{x}$ gives the desired feasible solution to $\lpconfigmin(\tilde{S} \cup \tilde{M})$ with objective value at most $\big(1 + O(\epsilon)\big) \opt \big( \lpconfigmin(S \cup \tilde{M}) \big)$.
\end{proof}

To summarize, on the sub-instance $\tilde{S} \cup \tilde{M}$, we can take $D = O(\frac{1}{\epsilon^2})$, because every medium job or block has size at least $\epsilon^2$, and $T = O(\frac{1}{\epsilon^3})$ by taking one type for each distinct medium job size and one type for the blocks of small jobs. It remains to assign the large jobs $L$ and use the blocks to assign the small jobs. This will give our complete algorithm.

\subsection{Putting it all together}

We combine the rounding for the configuration LP, the algorithm to realize a collection of configurations by an edge assignment, and the grouping/rounding operations for the jobs to define our complete algorithm guaranteed by \Cref{thm_main_off_min}.

\medskip
\hrule
\smallskip
\hrule
\smallskip
\minoffalg: Given collection $J$ of jobs and failover capacity $B \geq 1$, we assign them to edges as follows:
\begin{enumerate}
	\item Construct the sets of small, medium, and large jobs $J = S \cup M \cup L$ as well as the blocks of small jobs and grouped medium jobs $\bar{S}$ and $\bar{M}$, respectively as in \Cref{sec_small_large_jobs}.
	\item For each large job, open a matching edge (two machines) for that job and assign it there.
	\item For the blocks and grouped medium jobs, we have $T = O(\frac{1}{\epsilon^3})$ and $D = O(\frac{1}{\epsilon^2})$, so we run the algorithm guaranteed by \Cref{thm_lpconfig_main} to obtain an assignment of $\tilde{S} \cup \tilde{M}$ into at most $\opt \big(\lpconfigmin(\tilde{S} \cup \tilde{M})\big) + O(\frac{1}{\epsilon^5}) + error$ machines. We open this many machines and use the above assignment as a template to actually assign $S$ and $M \setminus L$
	\item Recall that we only increased the size of each job from $M \setminus L$ to $\tilde{M}$, so we can assign each job in $M \setminus L$ in the place of its corresponding job in $\tilde{M}$.
	\item For the jobs in $S$, we consider them in arbitrary order. When considering a job $j \in S$, if there exists a block in the template assignment with less than $\epsilon - s_j$ units of small jobs assigned there, then assign job in this block. If no such block exists, then we assign all remaining small jobs using \Cref{lem_matching_unit}.
\end{enumerate}
\medskip
\hrule
\smallskip
\hrule
\medskip

\begin{proof}[Proof of \Cref{thm_main_off_min}]
	It is immediate that \minoffalg~ is efficient and assigns all jobs. Further, this assignment satisfies the normal- and failover constraints: we put each large job on its own matching edge, our template assignment of $\tilde{S} \cup \tilde{M}$ is feasible by \Cref{thm_lpconfig_main}, we only assign smaller jobs in $S \cup M$ than in the template, and our assignment of the remaining small jobs is feasible by \Cref{lem_matching_unit}.
	
	It remains to show that the number of machines used is at most $\big(1 + O(\epsilon)\big) \opt \big( \lpconfigmin(J) \big) + O(\frac{1}{\epsilon^5})$ (recall by \Cref{lem_lpconfigmin_relax}, we have $\opt \big( \lpconfigmin(J) \big) \leq \opt(J)$.)  We handle the large, medium, and small jobs separately.
	
	\begin{enumerate}
		\item For the large jobs, we open $O(\lvert L \rvert)$ machines, where $\lvert L \rvert \leq \epsilon^3 \lvert M \rvert$ and every job in $M$ has size at least $\epsilon^2$. Note that every feasible configuration has at most $\frac{1}{\epsilon^2}$ medium jobs. Thus, $\lvert L \rvert \leq \epsilon^3 \lvert M \rvert \leq \epsilon^3 \frac{1}{\epsilon^2} \cdot  \opt \big( \lpconfigmin(J) \big) = \epsilon \cdot \opt \big( \lpconfigmin(J) \big)$. Thus we open $O(\epsilon) \cdot \opt \big( \lpconfigmin(J) \big)$ machines for the large jobs.
		\item For the medium jobs, our template assignment of $\tilde{S} \cup \tilde{M}$ opens $\opt \big(\lpconfigmin(\tilde{S} \cup \tilde{M})\big) + O(\frac{1}{\epsilon^5}) + error \leq \big(1 + O(\epsilon)\big) \opt \big( \lpconfigmin(J) \big) + O(\frac{1}{\epsilon^5}) + error$, using \Cref{lem_small_med_lp}. We assign all medium jobs in these machines.
		\item For the small jobs, it suffices to bound the number of extra machines needed for the remaining small jobs that do not fit in the blocks. Consider the first time that we consider a small job that cannot be assigned to any block. It must be the case that each block is already assigned at least $(\epsilon - \epsilon^2)$ units of small jobs. Recall that the number of blocks is $\lceil \frac{1}{\epsilon} \sum_{j \in S} s_j \rceil$. Thus the total size of already assigned small jobs is at least $(\epsilon - \epsilon^2) \lceil \frac{1}{\epsilon} \sum_{j \in S} s_j \rceil \geq (1 - \epsilon) \sum_{j \in S} s_j$. We conclude, the total size of remaining unassigned small jobs is at most $\epsilon \sum_{j \in S} s_j = O(\epsilon) \cdot \opt \big( \lpconfigmin(J) \big)$, which requires $O(\epsilon) \cdot \opt \big( \lpconfigmin(J) \big)$ machines by \Cref{lem_matching_unit}.
	\end{enumerate}
	Combining the machines from all three types of jobs gives the desired bound.
\end{proof}


==> stochastic-new.tex <==

	\section{Sublinear approximation in the stochastic model} \label{sec:stoch}
	
	We now consider \problem in the \emph{online stochastic model}, where, instead of being adversarial, the size $S_t$ of each demand now comes independently from an \emph{unknown} distribution $\mu$ over $[0,\min\{1,\frac{B}{2}\}]$. Again, at time $t$ the algorithms observes the size $S_t$ of the current demand and irrevocably assigns it to one of the $m$ machines. We still use $\OPT =  \OPT(S_1,\ldots,S_n)$ to denote the optimal value of the instance, which is now a random quantity. 
	
	The main result of this section is an algorithm that achieves a sublinear additive loss compared to the offline optimal solution in this stochastic model. As remarked above\mnote{do remark} such guarantees as impossible in the worst-case model. \mnote{Say somewhere (prelims?) that $O(X)$ just means that there is a constant such that $\le cst \cdot X$}
	
	\begin{thm} \label{thm:stoch}
		With probability at least $1 - O(\frac{1}{m})$, the total value of the algorithm \red{XX} is at least $\OPT - O(\OPT^{5/6} \log \OPT)$.
	\end{thm}
	
	The algorithm relies on a learn-and-pack approach which uses previously seen items to compute a \emph{template} for packing the next items. A crucial component for matching the new items to the ``template items'' are \emph{monotone matchings}.
	
	\begin{definition}[Monotone matching]
		\mnote{Define it: given two sequences, \ldots.}
	\end{definition}
	
	A surprising result of Rhee and Talagrand~\cite{xx} is that if the sequences are sampled iid from the same distribution, then almost all items can be matched, and moreover such matching can be found online (see~\cite{xx} for a more general result where the sequences may come form different distributions). 
	
	\begin{thm}[Monotone matching Theorem] \label{thm:rheeTal}
		Suppose the random variables $A_1,\ldots,A_n$ and $B_1,\ldots,B_n$ are all sampled independently from a distribution $\mu$. Then with probability at least $1 - e^{-cst \cdot \log^{3/2} n}$ there is a matching of the variables $A_t$'s to the $B_t$'s (we use $\pi$ to denote this matching, namely $A_t$ is matched to $B_{\pi(t)}$, or to no one if $\pi(t) = \emptyset$) such that:
		%
		\begin{enumerate}
			\item The matched pair is at least the original guy, namely $B_{\pi(t)} \ge A_t$ for all matched $t$
			
			\item Almost all $A_t$'s are matched, namely at most $cst \cdot \sqrt{n} \log^{3/4} n$ of them are unmatched. 
		\end{enumerate}
		Moreover, this matching can be computed even if the variables $A_t$'s come online. 
	\end{thm}
	
	
	\mnote{One thing is that we are hiding is that the constant in the $O(\cdot)$ depends on the distribution $\mu$, which is not ideal}
		
	
	\medskip
	\textbf{Main algorithm:}
	
	\medskip
	Repeatedly calls the procedure OneRound below, passing to it the number of machines still available/unopened (e.g. initially it calls $\oneround(m)$); it does this for $\frac{\log m}{\log 4/3}$ rounds. 
	
%it stops calling the subroutine whenever the number of available machines is at less than $8 (2 + 3 C \cdot f(\bar{n}))$ \red{[M: Actually also stop if has less than $2m^{5/6}$ machines left, algo will stop in first phase anyway]} or less than $100 \sqrt{n} + 2 + \frac{4}{\delta}$ (see Lemma \ref{lemma:openCst} for the definition of the $\bar{n}$, which should be just a constant, $C$ is just the constant from \Cref{thm:converges}, and $\delta$ is some constant that controls the probability of success). 
	

	
	\bigskip
	\textbf{OneRound($\tilde{m}$):}
	\medskip
	
	This is based on Rhee-Talagrand. 	It is convenient to rename the demands and use $Y_i$ to denote the $i$th demand seen by \oneround (which are still sampled iid from $\mu$). Each phase $k$ will see the previous $n_k := 2^k$ items, make a template based on them, and use it for the next $n_k$ items. It receives the number $\tilde{m}$ of machines that it can open, and never opens more than that. More precisely, consider the offline problem of minimizing the machines required to schedule all the demands $x_1,\ldots,x_n$. Consider the approximation algorithm from Section \ref{sec_offline_min_machines} for this offline problem, and let $\overline{\mach}(x_1,\ldots,x_n)$ be the number of machines it uses. (It may be useful to keep in mind that this algorithm achieves a sublinear approximation guarantee.) The algorithm \oneround is then:
	
	\begin{enumerate}
		\item Put the first item $Y_1$ on an edge by itself, opening 2 machines
		
		\item For phases $k = 0,1,2,\ldots$
		
		\begin{enumerate}
		\item See the first $n_k$ items $Y_1,\ldots,Y_{n_k}$. Run the algorithm from Section \ref{sec_offline_min_machines} to find a solution for them that uses $\overline{\mach}(Y_1,\ldots,Y_{n_k})$ machines; let $templ(t)$ denote the pair of machines that $Y_t$ is assigned to. This solution is our template.
		
		\item If $$\textrm{\#\,already open machines} + \underbrace{\overline{\mach}(Y_1,\ldots,Y_{n_k})}_{\textrm{\it machines from template}} + 2\cdot \underbrace{\cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k}_{\textrm{\it predicted unmatched demand}} + 2 m^{5/6} \,>\, \tilde{m},$$ then STOP
		%call the algorithm recursively (giving it $\tilde{m} - \textrm{[number of open machines]}$) to handle all the remaining items $X_{n_k + 1}, X_{n_k + 2},\ldots,X_n$
		
		\item Else, open a clique with $\overline{\mach}(Y_1,\ldots,Y_{n_k})$ machines. See the next $n_k$ demands $Y_{n_k + 1}, \ldots, Y_{2n_k}$ and assign them to machines based on the template using Rhee-Talagrand matching. 
		
		More precisely, find the Rhee-Talagrand monotone matching $\pi$ from Theorem \ref{thm:rheeTal} between the new and old demands and to every new matched demand $Y_t$ send it to machine that $Y_{\pi(t)}$ occupied in the template, namely the $templ(\pi(t))$-th newly opened machine. 
		
		Whichever demands cannot be matched to the template, put on an edge by itself (opening 2 more machines for each). If run out of machines, declare FAIL	
		\end{enumerate}
	\end{enumerate}
	
	\mnote{Say at some point around here that there are 2 important components that we postpone to their own sec.: Finding an almost optimal min number of machines, and the speed of convergence of this expected cost}
	We assume that $m$ is at least a sufficiently large constant, else the results trivially holds.\mnote{This is used in Claim \ref{claim:MU} for example. See exactly where to state this assumption, when to recall it, etc.} The core of the analysis is that \oneround gets good value density, i.e., the ratio value/machine. We use $\E S_0$ to denote the expected value of the size of a demand (which is the same as $\E S_t$ for any $t$). From \Cref{thm:converges}, we basically get that \OPT is able to fit roughly $\frac{1}{c(\mu)}$ demands per machine, and each such demand gives value roughly $\E S_0$; so the best possible density value/machine should be around $\frac{\E S_0 }{c(\mu)}$. We first make this formal in the next lemma. 
	
	\begin{lemma} \label{lemma:stochDensityOPT}
		With probability at least $1 - \frac{2}{m^2}$ we have $$\OPT \le m \cdot \frac{\E S_0}{c(\mu)} + O(m^{5/6}).$$
	\end{lemma}
	
	Crucially, the next lemma says that \oneround almost achieves this density.\mnote{Can we make the term $O(m^{5/6})$ slightly smaller, so that it times $\log m$ is at most $O(m^{5/6})$? Would clean up the bounds a bit}
		
	\begin{lemma} \label{lemma:stochDensity}
		Let $Open$ be the number of machines open by $\oneround(\tilde{m})$ (which is a random variable). Then with probability at least $1 - \frac{1}{m}$, the total value of the demands scheduled by $\oneround(\tilde{m})$ is at least $$\textrm{value of $\oneround(\tilde{m})$} \ge \frac{\E S_0}{c(\mu)} \cdot Open - O(m^{5/6}).$$ 
	\end{lemma}
	
	Given this lemma, we see that the total value of the main algorithm (which repeatedly calls \oneround) is approximately $\frac{\E S_0}{c(\mu)}$ times the total machines opened during the execution. We finally show that the number of opened machines is $\approx m$, thus almost matching the upper bound on \OPT from Lemma \ref{lemma:stochDensityOPT}.
		
%	Since there are is the loss $O(m^{5/6}$) in value in each call of OneRound, we also need to show that the main algorithm makes few calls to OneRound. The intuition is that OneRound should consume at least a constant fraction of the available machines $\tilde{m}$ before entering the phase where it STOPS/FAILS due to lack of machines. Then each call reduces the number of available machines my a constant factor, and so there are at most $\log m$ calls. 
	
	\begin{lemma} \label{lemma:stochLogCalls}
		With probability $1 - O(\frac{1}{m})$, the main algorithm opens at least $m - 5 \cstg \cdot m^{5/6}$ machines (where $\cstg$ is the constant from Lemma \ref{lemma:openCst}).
	\end{lemma}
	
	Before proving these lemmas we show how they imply Theorem \ref{thm:stoch}.\mnote{Since it is straightforward, could just give a proof sketch or omit it from the body}
	
	\begin{proof}[Proof of Theorem \ref{thm:stoch}]
	Let $L$ be the number of calls to \oneround that the main algorithm makes (which is a random variable), and let $val_i$ and $Open_i$ be the value obtained and number of machines opened by the $i$-th call. By Lemma \ref{lemma:stochLogCalls}, with probability at least $1 - \frac{1}{m^2}$ the number of call $L$ is at most $\cste \cdot \log m$; then employing Lemma \ref{lemma:stochDensity} on these at most $\cste \cdot \log m$ calls we have that with probability at least $1 - \frac{1 + \cste \cdot \log m}{m^2}$ the total value of the main algorithm is
	%
	\begin{align*}
		\textrm{algo value} ~=~ val_1 + \ldots + val_L ~\ge~ \frac{\E S_0}{c(\mu)} \cdot \sum_{i \le L} Open_i \,-\,O(m^{5/6} \log m).
	\end{align*}
	Moreover, from Lemma \ref{lemma:stochLogCalls}, with probability at least $1-O(\frac{1}{m})$ we have that the total number of machines open $\sum_{i \le L} Open_i$ is at least $m - 5 \cstg \cdot m^{5/6}$. Thus, the previous bound on the main algorithm's value becomes  
	%
	\begin{align*}
		\textrm{algo value} ~\ge~ m\cdot \frac{\E S_0}{c(\mu)} \,-\,O(m^{5/6} \log m).
	\end{align*}
	Furthermore, from Lemma \ref{lemma:stochDensityOPT} we have that $\OPT \le m \cdot \frac{\E S_0}{c(\mu)} + O(m^{5/6})$ with probability at least $1 - \frac{2}{m^2}$. So by taking a union bound and combining this the the above lower bound on the algorithm's value we get that with probability $1 - O(\frac{1}{m})$
	%
	\begin{align*}
		\textrm{algo value} ~\ge~ \OPT \,-\,O(m^{5/6} \log m) ~\ge~ \OPT - O(\OPT^{5/6} \log \OPT),
	\end{align*}		
	the last inequality following from the fact that $\OPT \le m$, since it can get at most 1 unit of value per machine\mnote{Double check $m$ vs $2m$}. This concludes the proof of Theorem \ref{thm:stoch}.
	\end{proof}	

	Now we prove Lemmas \ref{lemma:stochDensityOPT}--\ref{lemma:stochLogCalls}.
	
%##########################################################################
%##########################################################################

	
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################

	\subsection{Proof of Lemma \ref{lemma:stochDensityOPT}}

	Let $\mach(s_1,\ldots,s_n)$ be the minimum number of machines needed to schedule the demands $s_1,\ldots,s_n$\mnote{Make clear that this is not just bin packing}. For proving this lemma, we need the observation that the bound from Theorem \ref{thm:converges} holds not only in expectation but with high probability (with a negligible additional loss). To see that, notice that the function $\mach(s_1,\ldots,s_n)$ had bounded differences: changing the size of any demand $i$ from $s_i$ to $s'_i$ (both in the range $\min\{1, \frac{B}{2}\}$) can change the minimum number of machines required by at most 2, i.e. $$|\mach(s_1,\ldots,s_i,\ldots,s_n) - \mach(s_1,\ldots,s'_i,\ldots,s_n)| \le 2,$$ since we can always schedule the demand $i$ on an edge by itself (using 2 new machines) if needed. Then as a consequence of McDiarmid's Inequality (Lemma \ref{lemma:mcDiarmid}) with $\alpha = \lambda \sqrt{T}$ we directly obtain the following.
	
	\begin{cor}	\label{cor:convergesWHP}
		For every $T$ we have $$\mach(S_1,\ldots,S_T) \,\in\, T \cdot c(\mu) \pm O(T^{5/6}) \pm \lambda \sqrt{T}$$ with probability at least $1 - 2e^{-\frac{\lambda^2}{2}}$.
%		There is a constant $\csta$ such that for every $T$ we have  $$\mach(S_1,\ldots,S_T) \,\in\, T \cdot c(\mu) \pm \csta \cdot T^{5/6} \pm \lambda \sqrt{T}$$ with probability at least $1 - 2e^{-\frac{\lambda^2}{2}}$.
	\end{cor}

	Then by essentially inverting this bound, we can upper bound how many demands are scheduled by the optimal solution $\OPT(S_1,\ldots,S_n)$ for our original problem. 

%M: Older cleaner version without delta, but it seems that now we need delta
%	\begin{lemma} \label{lemma:numScheduled}
%		Consider the original problem \problem with $m$ machines. With probability at least $1 - \frac{1}{\delta}$ the optimal solution to the instance $S_1,\ldots,S_n \sim \mu$ schedules at most $\frac{m}{c(\mu)} + O(m^{5/6})$ demands. 
%	\end{lemma}
%
%	\begin{proof}[Proof sketch]
% Using Corollary \ref{cor:convergesWHP} with $\lambda = 2 \sqrt{\log m}$, one can see that there is a positive constant $d$ such that with probability at least $1-\frac{2}{m^2}$
%	%
%	\begin{align}
%	\mach(S_1,\ldots,S_T) \,\ge\, T \cdot c(\mu) - d^{5/6} \cdot T^{5/6} \label{eq:numScheduled}
%	\end{align}
%	for every number of demands $T \ge \log^{3/2} m$. 
%	
%	A bit of algebra shows that there is a value $\bar{T} = \frac{m}{c(\mu)} + O(m^{5/6})$ such that the right-hand side of \eqref{eq:numScheduled} is at least strictly more than $m$; in fact, taking $$\bar{T} := \max\bigg\{\frac{1}{c(\mu)}\bigg(m + \bigg(\frac{m (d+1)}{c(\mu)}\bigg)^{5/6}\bigg)\,,\, \frac{(d+1)\, d^{5/6}}{c(\mu)}\,,\, \log^{3/2} m \bigg\} + 1$$ suffices, which can be verified by applying the contrapositive of Lemma \ref{xx} presented in the appendix). This means that with probability at least $1-\frac{2}{m^2}$, the demands $S_1,\ldots,S_{\bar{T}}$ cannot all be scheduled within $m$ machines; in such scenarios the optimal solution then schedules at most $\bar{T} - 1 = \frac{m}{c(\mu)} + O(m^{5/6})$ demands, as claimed.  
%	\end{proof}
	
	\begin{lemma} \label{lemma:numScheduled}
		Consider the original problem \problem with $m$ machines. For every $\delta > 0$, with probability at least $1 - \delta$ the optimal solution to the instance $S_1,\ldots,S_n \sim \mu$ schedules at most $\frac{m}{c(\mu)} + O(m^{5/6}) + \log \frac{1}{\delta}$ demands. 
	\end{lemma}
	
	\begin{proof}[Proof sketch]
 Using Corollary \ref{cor:convergesWHP} with $\lambda = \sqrt{2 \log \frac{1}{2 \delta}}$, one can see that there is a positive constant $d$ such that with probability at least $1-\delta$
	%
	\begin{align}
	\mach(S_1,\ldots,S_T) \,\ge\, T \cdot c(\mu) - d^{5/6} \cdot T^{5/6} \label{eq:numScheduled}
	\end{align}
	for every number of demands $T \ge \log \frac{1}{\delta}$. 
	
	A bit of algebra shows that there is a value $\bar{T} = \frac{m}{c(\mu)} + O(m^{5/6}) + \log \frac{1}{\delta}$ such that the right-hand side of \eqref{eq:numScheduled} is strictly more than $m$ (the term $+\log \frac{1}{\delta}$ being present just to ensure $\bar{T} \ge \log \frac{1}{\delta}$); in fact, taking $$\bar{T} := \max\bigg\{\frac{1}{c(\mu)}\bigg(m + \bigg(\frac{m (d+1)}{c(\mu)}\bigg)^{5/6}\bigg)\,,\, \frac{(d+1)\, d^{5/6}}{c(\mu)}\,,\, \log \frac{1}{\delta} \bigg\} + 1$$ suffices, which can be verified by applying the contrapositive of Lemma \ref{xx} presented in the appendix). This means that with probability at least $1-\frac{2}{m^2}$, the demands $S_1,\ldots,S_{\bar{T}}$ cannot all be scheduled within $m$ machines; in such scenarios the optimal solution then schedules at most $\bar{T} - 1 = \frac{m}{c(\mu)} + O(m^{5/6}) + \log \frac{1}{\delta}$ demands, as claimed.  
	\end{proof}
	
	We can now show that with high probability $\OPT(S_1,\ldots,S_n) \le m \cdot \frac{\E S_0}{c(\mu)} + O(m^{5/6})$ and concludes the proof of Lemma \ref{lemma:stochDensityOPT}. Setting $\delta = \frac{1}{m^2}$ and letting $\bar{T} = \frac{m}{c(\mu)} + O(m^{5/6})$ be the above upper bound on the number of demands scheduled by $\OPT(S_1,\ldots,S_n)$, with probability $\ge 1 - \frac{1}{m^2}$ we have that $\OPT(S_1,\ldots,S_n) \le \sum_{t \le \bar{T}} S_t$. Moreover, employing the Chernoff bound (Lemma \ref{lemma:chernoff}) with $\lambda = \sqrt{\bar{T} \log m}$, with probability at least $1- \frac{1}{m^2}$ this sum can be upper bounded as 
	%
	\begin{align*}
		\sum_{t \le \bar{T}} S_t \,\le\, \bar{T} \cdot \E S_0 + \sqrt{\bar{T} \log m} \,\le\, m \cdot \frac{\E S_0}{c(\mu)} + O(m^{5/6}). 
	\end{align*}
	Taking a union bound to combine the two previous bounds, with probability at least $1 - \frac{2}{m^2}$ we have that $\OPT(S_1,\ldots,S_n) \le  m \cdot \frac{\E S_0}{c(\mu)} + O(m^{5/6})$, as desired. This concludes the proof of the Lemma \ref{lemma:stochDensityOPT}. 

%#########################################################################
%#########################################################################

	\subsection{Proof of Lemma \ref{lemma:stochDensity}} 

	First, we control in high-probability the number of phases that $\oneround(\tilde{m})$ executes before stopping or failing; this will be important to avoid dependencies on the total number of demands $n$ in the instance, which can be arbitrarily bigger than the scale of the effective instance. 

	\begin{claim} \label{claim:numPhases}
		With probability at least $1 - \frac{1}{m^2}$ the algorithm \oneround performs at most 
	%
	\begin{align}
	\bar{k} := \log \bigg(\frac{\tilde{m}}{c(\mu)} + O(\tilde{m}^{5/6}) + 2\log m\bigg) \label{eq:barK}
	\end{align}
	phases.
	\end{claim}

	\begin{proof}
	Recall that the demands sizes $Y_1,Y_2,\ldots$ that \oneround sees are still iid samples from the original distribution $\mu$. Then using Lemma \ref{lemma:numScheduled} with $m=\tilde{m}$, we get that with probability at least $1 - \frac{1}{m^2}$ \oneround can schedule at most $\frac{\tilde{m}}{c(\mu)} + O(\tilde{m}^{5/6}) + 2 \log m$ many of these demands; this implies that it either stops or fails by round $\bar{k}$.
	\end{proof}	
	
	Next, we need to bound how many machines are open by \oneround, which in particular affects the probability of it FAILing. For a phase $k$, let $M_k := \overline{\mach}(Y_1,\ldots,Y_{n_k})$ denote the number of machines in the template solution, and let $U_k$ be the number of additional machines that had to be open to accommodate the unmatched demands among $Y_{n_k +1},\ldots,Y_{2n_k}$, namely twice the number of unmatched items. Notice that these quantities are well defined even for phases that the algorithm did not execute. The quantity $M_k + U_k$ is then the number machines that the algorithm \oneround opens in phase $k$ (if it executes it). We have the following bounds for the number of bins open, at least for a phase $k$ where the number of items $n_k$ is sufficiently large (but still sublinear in $m$).
	
	\begin{claim} \label{claim:MU}
	  Let $k_0 := (\frac{2}{\cstc} \log m)^{2/3}$. Then there is a constant $\csta$ such that:
	  \begin{enumerate}
	  	\item For $k \ge k_0$, we have $M_k \,\in\, n_k \cdot c(\mu) \,\pm\, 2 \csta \cdot n_k^{5/6}$ with probability $\ge 1 - \frac{1}{m^2}$
	  	
	  	\item For $k \ge k_0$, we have $U_k \le 2 \cstb \cdot \sqrt{n_k}\,\log^{3/4} n_k$\mnote{Change $\cstb$ to $\csta$, there's no reason to use diff constants now} with probability $\ge 1 - \frac{1}{m^2}$
	 		\item $n_{k_0} \le m^{5/6}$.
		\end{enumerate}
	\end{claim}
	
	\begin{proof}
	 Consider a phase $k \ge k_0$. First, from the guarantee of the algorithm for \red{XXX} \mnote{Name of the offline min problem} used to build the template (Theorem \ref{thm_main_off_min} with $\e = n_k^{1/3}$), we have that $$\mach(Y_1,\ldots,Y_{n_k}) \,\le\, M_k \,\le\, \mach(Y_1,\ldots,Y_{n_k}) + O(n_k^{5/6}).$$ Since the demand sizes $Y_1,\ldots,Y_{2n_k}$ seen in this phase are iid samples from the original distribution $\mu$, we can use Corollary \ref{cor:convergesWHP} with $\lambda = n_k^{1/3}$ to further bound the number of machines $M_k$ as 
	 %
	 \begin{align*}
	 	M_k \,&\in\, n_k \cdot c(\mu) \pm \csta \cdot n_k^{5/6}
	 \end{align*}
	 with probability at least $1 - 2e^{-\frac{n_k^{2/3}}{2}}$ for some constant $\csta$. But since $n_k = 2^k \ge 2^{k_0}$, a quick calculation show that this probability is at least $1 - \frac{1}{m^2}$\mnote{We are assuming $\cstc$ is suff small, else increase a bit $k_0$}, proving the first item of the claim.  	 

	 To control $U_k$, we can use the Monotone Matching Theorem (Theorem \ref{thm:rheeTal}) with the first sequence of sizes being the demands from the template, i.e., $(A_1,\ldots,A_{n_k}) = (Y_1,\ldots,Y_{n_k})$, and the second one being the demands that we attempted to match to them, namely $(B_1,\ldots,B_{n_k}) = (Y_{n_k+1}, \ldots,Y_{2n_k})$ to obtain that the number of unmatched demands it at most $\cstb \cdot \sqrt{n_k}\,\log^{3/4} n_k$ with probability at least $1- e^{-\cstc \cdot \log^{3/2} n_k}$, and hence with this probability
 	 %
	 \begin{align*}
	 	U_k \,\le\, 2 \cstb \cdot \sqrt{n_k}\,\log^{3/4} n_k.
	 \end{align*}
	Again because\ $k \ge k_0$, we get that this probability is at least $1- \frac{1}{m^2}$, proving Item 2 of the claim. 
	
	The last item $n_{k_0} \le m^{5/6}$ of the claim follows can be directly verified using the fact that we assumed $m$ is at least a sufficiently large constant. 
	\end{proof}
	 
	Recall that \oneround only FAILs when the number of machines $M_k + U_k$ actually opened in a phase is bigger than it ``predicted'' in Line \ref{xx}, and this prediction is exactly $M_k$ plus the upper bound $U_k$ from Claim \ref{claim:MU} plus a slack of $2 m^{5/6}$. By considering all phases, it is now easy to upper bound the probability that \oneround FAILs.
	
	\begin{claim} \label{claim:failPr}
	The probability that \oneround fails is at most $\frac{\bar{k} + 1}{m^2}$.
	\end{claim}
	
	\begin{proof}
Fix any phase $k$, and we claim that the probability that \oneround FAILs on this phase is at most $\frac{1}{m^2}$. If \oneround FAILSs on phase $k$, then it did not STOP in Line \ref{xx}, so $$\textrm{\#\,[machines open before phase $k$]} + \overline{\mach}(Y_1,\ldots,Y_{n_k}) + 2 \cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k + 2m^{5/6} ~\le~ \tilde{m},$$ but it ran out of machines during phase $k$, namely  $$\textrm{\#\,[machines open before phase $k$]} + (M_k + U_k) > \tilde{m}.$$ Since $M_k = \overline{\mach}(Y_1,\ldots,Y_{n_k})$, these observations imply that $U_k > 2 \cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k + 2m^{5/6}$. This is impossible if $n_k \le m^{5/6}$, because the number of machines $U_k$  opened for the unmatched demands is always at most twice the number $n_k$ of demands considered for the matching. So we must have $n_k > m^{5/6}$ (and so from Claim \ref{claim:MU} $k \ge k_0$) and at least $U_k > 2\cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k$; but again by Claim \ref{claim:MU} the latter happens with probability at most $\frac{1}{m^2}$. Thus, the probability that \oneround fails on phase $k$ is at most $\frac{1}{m^2}$.

	Moreover, by Claim \ref{claim:numPhases}, with probability at least $1- \frac{1}{m^2}$ \oneround has at most $\bar{k}$ phases. Then taking a union bound, we see that the event that \oneround has at most $\bar{k}$ phases and in all of them it does not fail holds with probability at least $1 - \frac{\bar{k} + 1}{m^2}$; in particular, with at least this much probability the algorithm does not fail in its execution, which proves the claim.
	\end{proof}
	 
	We now finally lower bound the value that \oneround gets. Let $\tau$ be the (random) index of the last phase attempted by \oneround, namely where Step \ref{xx}\mnote{(c)} is executed. As long as it does not FAIL on the last phase $\tau$ (which by the previous claim happens with probability at least $1 - \frac{\bar{k}+1}{m^2}$) \oneround gets the value of all items up until this phase, that is
	%
	\begin{align}
	\textrm{value of \oneround} \,\ge\, Y_1 + \ldots + Y_{2n_\tau} \,\ge\, Y_1 + \ldots + Y_{2n_{\blue{\min\{\tau,\bar{k}\}}}}.  \label{eq:valOneRound}
	\end{align}
		Recall that the $Y_i$'s are independent and each has mean $\E S_0$. Then employing the Chernoff bound with $\lambda = \sqrt{n_{\bar{k}} \log (m^2 \cdot n_{\bar{k}})}$, for any fixed $t \le n_{\bar{k}}$ we have that 
	 %
	 \begin{align*}
	 Y_1 + \ldots + Y_t \ge t \cdot \E S_0 - \sqrt{n_{\bar{k}} \log (m^2 \cdot n_{\bar{k}})} ~~~~~~\textrm{with probability at least $1 - \frac{1}{m^2 \cdot n_{\bar{k}}}$}.
	 \end{align*}
	 Then taking a union bound over \eqref{eq:valOneRound}, the previous displayed inequality for all $t \le n_{\bar{k}}$, and over the event that \oneround has at most $\bar{k}$ phases (which holds with probability at least $1- \frac{1}{m^2}$) we get that \mnote{Set $\delta'$ so that $\delta' (\bar{k}+1) \le \frac{1}{m^2}$}
	%
	\begin{align}
	\textrm{value of \oneround} \,&\ge\, 2n_{\min\{\tau,\bar{k}\}} \cdot \E S_0 - \sqrt{n_{\bar{k}} \log (m \cdot n_{\bar{k}})}\notag\\
	&= 2n_\tau \cdot \E S_0 - \sqrt{n_{\bar{k}} \log (m \cdot n_{\bar{k}})}\notag\\
	&\ge 2n_\tau \cdot \E S_0 - O(m^{5/6}) ~~~~~~~~~~~~\textrm{with probability $\ge 1 - \frac{\bar{k} + 3}{m^2}$}.   \label{eq:valOneRound2}
	\end{align}	 
	 
	To conclude the proof of Lemma \ref{lemma:stochDensity} we just need to relate this quantity to the number of machines opened by \oneround. Let $Open_\ell$ be the number of machines opened until (including) phase $\ell$, and recall that $Open$ is the number of machines opened over all phases. Since the number of machines opened on phase $k$ is $M_k + U_k$ (plus two machines for the first demand $Y_1$), we have 
	%
	\begin{align}
	Open_\ell = 2 + (M_1 + U_1) + \ldots + (M_\ell + U_\ell)  \label{eq:openEll}%~~~~~~\textrm{with probability $\ge 1 - \frac{1}{m^2}$}. 
	\end{align}
%{\min\{\tau,\bar{k}\}}

	To upper bound the right-hand side, for the phases $k < k_0$ we just use the fact that $M_k + U_k \le 2n_k + 2n_k = 4n_k$, since both in the template and for the unmatched demands we never open more than 2 machines per demand considered (and $n_k$ demands are considered in each part). For a each phase $k = k_0, \ldots, \bar{k}$ we can use Claim \ref{claim:MU} to upper bound $M_k + U_k$ with probability at least $1 - \frac{2}{m^2}$ by
	%
	\begin{align*}
	M_k + U_k &\le n_k \cdot c(\mu) + 2 \csta \cdot n_k^{5/6} + 2 \cstb \cdot \sqrt{n_k}\,\log^{3/4} n_k\\
	&\le n_k \cdot c(\mu) + \cstd \cdot n_k^{5/6}
	\end{align*}
	for some constant $\cstd$. Together these bounds give that with probability at least $1 - \frac{2\ell}{m^2}$
	%
	\begin{align*}
	Open_\ell &\le 2 + \sum_{k < k_0} 4 n_k + \sum_{k = k_0}^{\ell} \bigg( n_k \cdot c(\mu) + \cstd \cdot n_k^{5/6} \bigg).
	\end{align*}	
	To further upper bound the first summation on the right-hand side, because of the exponential relationship $n_k = 2^k$, we have $\sum_{k < k_0} 4n_k \le 8 n_{k_0 - 1} \le O(m^{5/6})$, the last inequality coming from Claim \ref{claim:MU}; for the second summation, we analogously have $\sum_{k=k_0}^{\ell} n_k \le 2 n_\ell$ and $\sum_{k = k_0}^{\ell} n_k^{5/6} \le O(n_{\ell}^{5/6}) \le O(m^{5/6})$. Therefore,
	%
	\begin{align}
	Open_\ell \,\le\, 2 n_\ell \cdot c(\mu) + O(n_{\ell}^{5/6}) + O(m^{5/6})~~~~~\textrm{with probability at least $1 - \frac{2\ell}{m^2}$}. \label{eq:openEll2}
	\end{align}
	Finally, since by Claim \ref{claim:numPhases}, the number of phases $\tau$ performed by \oneround is at most $\bar{k}$ with probability at least $1 - \frac{1}{m^2}$, the total number of machines open can be upper bounded  
	%
	\begin{align*}
		Open \,\le\, Open_{\min\{\tau,\bar{k}\}} \,\le\, 2 n_{\tau} \cdot c(\mu) + O(n_{\bar{k}}^{5/6}) + O(m^{5/6}) \,\le\, 2 n_{\tau} + O(m^{5/6})
	\end{align*}
	with probability at least $1 - \frac{2 \bar{k} + 1}{m^2}$. 
	
		Finally, taking a union bound to combine this inequality with \eqref{eq:valOneRound2} we get that 
	%
	\begin{align*}
		\textrm{value of \oneround} &\,\ge\, \frac{\E S_0}{c(\mu)} \cdot Open - O(m^{5/6})
	\end{align*}
	with probability at least $1 - \frac{3 \bar{k} + 4}{m^2}$. Since $m$ is at least a sufficiently large constant, we have $m \ge 2\bar{k} + 1$, and the bound from the displayed inequality holds with probability at least $1 - \frac{1}{m}$. This proves Lemma \ref{lemma:stochDensity}.

%########################################################################
%########################################################################

	\subsection{Proof of Lemma \ref{lemma:stochLogCalls}}	
	
	To prove Lemma \ref{lemma:stochLogCalls} it will suffice to show that with high probability \oneround consumes a quarter of the machines available, unless there are already few machines available. 
		
	\begin{lemma} \label{lemma:openCst}
		There is a constant $\cstg$ such that whenever $\tilde{m} \ge 4 \cstg \cdot m^{5/6} + 8$, we have that $\oneround(\tilde{m})$ opens at least $\frac{\tilde{m}}{4}$ machines with probability at least $1 - \frac{\log(m/c(\mu))}{m^2}$.   
	\end{lemma}	

	\begin{proof}
	The main element of the proof is a converse to Claim \ref{claim:numPhases}, that is, a lower bound on the number of phases performed by \oneround. To argue that it has not ran out of machines on an initial phase, let $UB_\ell$ be the upper bound on the number of machines opened by the \oneround until phase $\ell$ given by \eqref{eq:openEll2}, namely $$UB_\ell = 2 n_\ell \cdot c(\mu) + \cstf \cdot n_{\ell}^{5/6} + \cstf \cdot m^{5/6}$$ for a sufficiently large constant $\cstf$. Here is the desired bound on the number of phases performed. 
	
		\begin{claim} \label{claim:LBPhases}
		Let $\underbar{k}$ be the largest integer $\ell$ such that $UB_\ell + 2 m^{5/6} \le \tilde{m}$. Then with probability at least $1 - \mubar{k}/m^2$ the algorithm $\oneround(\tilde{m})$ performs at least $\mubar{k}$ phases. 
	\end{claim}
	
	\begin{proof}
	\mnote{This claim could be streamlined, feels clunky} 
	From \eqref{eq:openEll2} and the fact that $\cstf$ is sufficiently large, we have with probability at least $1-\mubar{k}/m^2$
	%
	\begin{align}
	Open_{\mubar{k}} \,+\, 2\cdot \cstb \cdot \sqrt{n_{\mubar{k}}}\, \log^{3/4} n_{\mubar{k}} \,\le\, UB_{\mubar{k}}\,. \label{eq:mubar}
	\end{align}
	Under this event we see that \oneround starts phase $\mubar{k}$, that is, it does not STOP in Step (b) in the beginning of this iteration, since at that point
	%
	\begin{align*}
&~~\textrm{\#\,already open machines} + \overline{\mach}(Y_1,\ldots,Y_{n_k}) + 2\cdot \cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k + 2 m^{5/6}\\
&= Open_{\mubar{k}-1} \,+\, M_k \,+\, 2\cdot \cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k + 2 m^{5/6}	\\
&\le Open_{\mubar{k}} \,+\, 2\cdot \cstb \cdot \sqrt{n_k}\, \log^{3/4} n_k \,+\, 2 m^{5/6}\\
&\le UB_{\mubar{k}} + 2m^{5/6} \le \tilde{m},
	\end{align*} 
	where the last inequality follows from the definition of $\mubar{k}$. Moreover, under this event the algorithm also does not run out of machines (i.e. FAILs) on this phase $\mubar{k}$, since again $Open_{\mubar{k}} \le UB_{\mubar{k}} \le \tilde{m}$. The claim then follows.
	\end{proof}

	Using this claim plus the lower bound on the number of machines $M_k$ open on a round $k$ from Claim \ref{claim:MU}, we have that with probability at least $1 - 2 \mubar{k}/m^2$
	%
	\begin{align}
		Open \ge Open_{\mubar{k}} \ge \sum_{k = k_0}^{\mubar{k}} M_k &\ge \sum_{k = k_0}^{\mubar{k}}  \bigg(n_k \cdot c(\mu) \,-\, 2 \csta \cdot n_k^{5/6}\bigg) \notag\\
		&\ge \sum_{k=1}^{\mubar{k}} n_k \cdot c(\mu) - \sum_{k=1}^{k_0} n_k \cdot c(\mu) - \sum_{k=1}^{\mubar{k}} 2 \csta \cdot n_k^{5/6}  \notag\\
		&\ge (2 n_{\mubar{k}} - 1)\,c(\mu) - 2 n_{k_0}  - 5 \csta \cdot n_{\mubar{k}}^{5/6} \notag \\
		&\ge (2 n_{\mubar{k}} - 1)\,c(\mu) - 2 m^{5/6}  - \frac{5 \csta}{c(\mu)^{5/6}} \cdot m^{5/6}, \label{eq:LBOpen}
	\end{align}
	where the next-to-last equality follows from the definition $n_k = 2^k$, and the last inequality uses Claim \ref{claim:MU} and that the definition of $\mubar{k}$ implies $n_{\mubar{k}} \le \frac{\tilde{m}}{c(\mu)} \le \frac{m}{c(\mu)}$.
	
 	To further lower bound this quantity, from the maximality of $\mubar{k}$ we have $UB_{\mubar{k}+1} + 2m^{5/6} > \tilde{m}$, which expanding the definition of $UB_{\mubar{k}+1}$ gives
 	%
 	\begin{align*}
 		2 n_{\mubar{k}} \cdot c(\mu) > \frac{1}{2} \bigg(\tilde{m} - \cstf \cdot n^{5/6}_{\mubar{k}+1} - (\cstf + 2) m^{5/6}\bigg) \ge \frac{\tilde{m}}{2} -\bigg(\frac{\cstf}{2 c(\mu)^{5/6}} + \frac{\cstf}{2} + 1\bigg)
 		m^{5/6}.
 	\end{align*}
 	Employing this on inequality \eqref{eq:LBOpen} we get that with probability at least $1- 2\mubar{k}/m^2$
 	%
 	\begin{align*}
 	Open \ge \frac{\tilde{m}}{2} - \underbrace{\bigg(\frac{\cstf/2 + 5 \csta }{c(\mu)^{5/6}} + \frac{\cstf}{2} + 3 \bigg)}_{=:\cstg}\, m^{5/6} - 2.
 	\end{align*}
	Under the assumption $\tilde{m} \ge 4 \cstg \cdot m^{5/6} + 8$ of Lemma \ref{lemma:openCst}, we get $Open \ge \frac{\tilde{m}}{4}$ as desired. To finalize, since $n_{\mubar{k}} \le \frac{m}{c(\mu)}$, we have $\mubar{k} \le \log \frac{m}{c(\mu)}$, and so this happens with probability at least $1 - \frac{m/c(\mu)}{m^2}$. This concludes the proof of Lemma \ref{lemma:openCst}. 
 \end{proof}
 
 We now turn to the proof of the main lemma. 
 
 \begin{proof}[Proof of Lemma \ref{lemma:stochLogCalls}]
 	We assume that $m$ is at least a sufficiently large constant, otherwise the directly hold (with an appropriate constant in the term $O(\frac{1}{m})$); in particular, we assume that $5 \cstg \cdot m^{5/6} \ge 4 \cstg \cdot m^{5/6} + 8$, which will be useful to clean up the bounds. 
 	
 	Let $\tilde{m}_i$ denote the number of unopened machines right before the $i$-th call to \oneround made by the main algorithm (i.e., at this call $\tilde{m}_i$ is the parameter passed to \oneround). Define the (bad) event $E_i$ that in the beginning of round $i$ we still have more than $5 \cstg m^{5/6}$ unopened machines but (unlike what is prescribed by Lemma \ref{lemma:openCst} above) we did not consume open at least a quarter of these machines, i.e.  
 	%
 	\begin{align*}
 		E_i \equiv (\tilde{m}_i > 5 \cstg \cdot  m^{5/6}) \textrm{ and } (\tilde{m}_{i+1} > \tfrac{3}{4} \tilde{m}_i).
 	\end{align*}
 	
 	We claim that when neither of the events $E_1,\ldots,E_{\bar{r}}$ holds (for $\bar{r} := \frac{\log m}{\log 4/3}$), then the total number of machines opened by the main algorithm is at least $m - 5 \cstg \cdot m^{5/6}$, which is what we want. To see this claim, notice that in this situation there are two cases:
 	
 	\paragraph{Case 1:} There is an event $E_i$ ($i \le \bar{r}$) which does not hold because $\tilde{m}_i \le 5 \cstg \cdot  m^{5/6}$. But this means that at the beginning of round $i$ the main algorithm has already opened $m - \tilde{m}_i \ge m - 5 \cstg \cdot  m^{5/6}$ machines, and the claim holds.
 	
 	\paragraph{Case 2:} All the events $\{E_i\}_{i \le \bar{r}}$ do not hold because $\tilde{m}_{i+1} \le \tfrac{3}{4} \tilde{m}_i$ for all of them. But this means that in beginning of the last round $\bar{r}$ there are $$\tilde{m}_{\bar{r}} \,\le\, (\tfrac{3}{4})^{\bar{r}} \cdot \tilde{m}_1 \,=\, (\tfrac{3}{4})^{\bar{r}}\cdot m \,=\, 1 \,\le\, 5 \cstg \cdot m^{5/6}$$ unopened machines, and so the claim also holds. 
 	
 	So to prove Lemma \ref{lemma:stochLogCalls} it suffices to show that the probability that an event $\{E_i\}_{i \le \bar{r}}$ holds is at most $O(\frac{1}{m})$. This probability is 
 	%
 	\begin{align}
 	\Pr\bigg(\bigvee_{i \le \bar{r}} E_i\bigg) \,\le\, \sum_{i \le \bar{r}} \Pr(E_i).  \label{eq:unionE}
 	\end{align}
 	To upper bound the right-hand side, we have $$\Pr(E_i) = \Pr(\tilde{m}_{i+1} > \tfrac{3}{4} \tilde{m}_i \mid \tilde{m}_i > 5 \cstg \cdot  m^{5/6}) \Pr(\tilde{m}_i > 5 \cstg \cdot  m^{5/6}).$$ But conditioning on $\tilde{m}_i > 5 \cstg \cdot  m^{5/6}$ (or more precisely, conditioning on the demands up to the beginning of round $i$ so that this event holds) and applying Lemma \ref{lemma:openCst} (notice that even with this conditioning the items within round $i$ are still sampled iid from $\mu$) we have that the first term in the right-hand side is at most $\frac{\log(m/c(\mu))}{m^2}$; so this gives $\Pr(E_i) \le \frac{\log(m/c(\mu))}{m^2}$. Employing this on \eqref{eq:unionE} gives 
  %
 	\begin{align*}
 	\Pr\bigg(\bigvee_{i \le \bar{r}} E_i\bigg) \,\le\, \bar{r} \cdot \frac{\log(m/c(\mu))}{m^2} \,=\, O\bigg(\frac{\log m}{m^2} \bigg) \,=\, O\bigg(\frac{1}{m} \bigg).
 	\end{align*}	
 	This concludes the proof of Lemma \ref{lemma:stochLogCalls}.  
 \end{proof}
